Internal entrainment and the origin of jet-related broad-band emission in Centaurus A

The dimensions of Fanaroff-Riley class I jets and the stellar densities at galactic centres imply that there will be numerous interactions between the jet and stellar winds. These may give rise to the observed diffuse and 'knotty' structure of the jets in the X-ray, and can also mass load the jets. We performed modelling of internal entrainment from stars intercepted by Centaurus A's jet, using stellar evolution- and wind codes. From photometry and a code-synthesised population of 12 Gyr (Z = 0.004), 3 Gyr (Z = 0.008) and 0 - 60 Myr (Z = 0.02) stars, appropriate for the parent elliptical NGC 5128, the total number of stars in the jet is ~ 8 x 10^8. Our model is energetically capable of producing the observed X-ray emission, even without young stars. We also reproduce the radio through X-ray spectrum of the jet, albeit in a downstream region with distinctly fewer young stars, and recover the mean X-ray spectral index. We derive an internal entrainment rate of ~ 2.3 x 10^-3 Msun yr^-1 which implies substantial jet deceleration. Our absolute nucleosynthetic yields for the AGB stellar population in the jet show the highest amounts for 4He, 16O, 12C, 14N and 20Ne. If some of the events at >= 55 EeV detected by the Pierre Auger Observatory originate from internal entrainment in Centaurus A, we predict that their composition will be largely intermediate-mass nuclei with 16O, 12C and 14N the key isotopes.

==> journals.tex <==
\bibpunct{(}{)}{;}{a}{}{,}
\def\aap{A\&A}                % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}              % Astronomy and Astrophysics, Supplement
\def\aj{AJ}                   % Astronomical Journal
\def\ajph{Australian J.~Phys.}% Australian Journal of Physics
\def\alet{Astro.~Lett.}       % Astronomical Letters
\def\ao{Applied Optics}       % Applied Optics
\def\apj{ApJ}                 % Astrophysical Journal
\def\apjl{ApJ}                % Astrophysical Journal, Letters
\def\apjs{ApJS}              % Astrophysical Journal, Supplement
\def\apss{Ap\&SS}             % Astrophysics and Space Science
\def\araa{ARA\&A}             % Annual Review of Astronomy and Astrophysics
\def\asr{Av.~Space Res.}     % Advances in Space Research
\def\azh{AZh}                 % Astronomiceskij Zhurnal
\def\baas{BAAS}               % Bulletin of the American Astronomical Society
\def\cpc{Comput.~Phys.~Commun.} % Computer Physics Communications
\def\gca{Geochim.~Cosmochim.~Acta} % Cheochimica et Cosmochimica Acta
\def\iaucirc{IAU Circ.}       % International Astronomical Union, Circular
\def\ibvs{IBVS}               % International Bulletin of Variable Stars
\def\icarus{Icarus}           % Icarus
\def\jcomph{J.~Comput.~Phys.} % Journal of Computational Physics
\def\jcp{J.~Chem.~Phys.}      % Journal of Chemical Physics
\def\jgr{J.~Geophys.~R.}      % Journal of Geophysical Research
\def\jrasc{JRASC}             % Journal of the RAS of Canada
\def\met{Meteoritics}         % Meteoritics
\def\mmras{MmRAS}             % Memoirs of the Royal Astronomical Society
\def\mnras{MNRAS}             % Monthly Notices of the RAS
\def\mps{Meteoritics and Planetary Science} % Meteoritics and Planetary Science
\def\nast{New Astron.}        % New Astronomy
\def\nat{Nature}              % Nature
\def\pasj{PASJ}               % Publ. of the Astronomical Society of Japan
\def\pasp{PASP}               % Publ. of the Astron. Society of the Pacific
\def\phr{Phys.~Rev.}          % Physical Review
\def\pdra{Phys.~Rev.~A}       % Physical Review A
\def\prb{Phys.~Rev.~B}       % Physical Review B
\def\prc{Phys.~Rev.~C}       % Physical Review C
\def\prd{Phys.~Rev.~D}       % Physical Review D
\def\phrep{Phys.~Rep.}        % Physics Reports
\def\phss{Phys.~Stat.~Sol.}        %
\def\procspie{Proc.~SPIE}     % Proceedings of the SPIE
\def\planss{Planet.~Space Sci.}  % Planetary & Space Sciences
\def\qjras{QJRAS}             % Quarterly Journal of the RAS
\def\rpph{Rep.~Prog.~Phys.}   % Reports on Progress in Physics
\def\rgsp{Rev.~Geophys.~Space Phys.~} % Reviews on Geophysics and Space Physics
\def\sal{Soviet Astron.~Lett.}% Soviet Astronomy Letters
\def\sci{Science}             % Science
\def\solph{Sol.~Phys.}        % Solar Physics
\def\ssr{Space Sci.~Rev.}     % Space Science Reviews
\def\zap{Z.~Astrophys.}       % Zeitschrift fuer Astrophysik

